Remote Monitoring of Two-State Markov Sources via Random Access Channels: an Information Freshness vs. State Estimation Entropy Perspective

We study a system in which two-state Markov sources send status updates to a common receiver over a slotted ALOHA random access channel. We characterize the performance of the system in terms of state estimation entropy (SEE), which measures the uncertainty at the receiver about the sources' state. Two channel access strategies are considered: a reactive policy that depends on the source behaviour and a random one that is independent of it. We prove that the considered policies can be studied using two different hidden Markov models and show through a density evolution analysis that the reactive strategy outperforms the random one in terms of SEE while the opposite is true for age of information. Furthermore, we characterize the probability of error in the state estimation at the receiver, considering a maximum a posteriori and a low-complexity (decode & hold) estimator. Our study provides useful insights on the design trade-offs that emerge when different performance metrics are adopted. Moreover, we show how the source statistics significantly impact the system performance.

==> dh.tex <==
\section{Pragmatic State Estimation: Decode\&Hold} \label{sec:dh}

The approach presented in Secs.~\ref{sec:optimumEstimation} and \ref{sec:de} allows to derive an analytical characterization of the SEE leaning on the APP logarithmic ratio $\lambda_n$. This quantity, in turn, combined with a threshold test ($\hat{x}_n=0$ if $\lambda_n>0$ and $\hat{x}_n=1$ otherwise), yields an optimum \ac{MAP} estimator, i.e, an estimator that minimizes the state estimation error probability introduced in \eqref{eq:Pe_def}. The complexity entailed by running a \ac{MAP} estimator may however be critical in many settings, e.g., when messages are delivered to a battery-powered and computationally-limited collector \cite{LoRa,Wang17_CommMag}. For such scenarios, other detectors may be preferred, trading off an optimal estimate in favor of a simpler implementation. 

Starting from this remark, we consider in this appendix an alternative solution, based on a \emph{decode and hold} (D\&H) estimator. Following this approach, the receiver maintains at any time $n$ an estimate $\est_n$ for the reference source, which is updated whenever a packet is decoded and reveals the current state of the node of interest, or remains unchanged otherwise. More formally:
\begin{align}
	\est_n = 
	\begin{cases}
		Y_n 		& \text{if } Y_n \in\{0,1\}\\
		\est_{n-1}	& \text{if } Y_n \in\{\idle,\collision,\izero,\ione\}\,.
	\end{cases}
\label{eq:DH_def}
\end{align}
As highlighted in \eqref{eq:DH_def}, the D\&H solution does not require the calculations of an APP logarithmic ratio as in the MAP estimator. On the other hand, the following example provides an intuition of why the simple scheme is inherently suboptimal.
\begin{example}
	Consider the case of a system with $M=2$ sources, operating under the reactive transmission strategy, and assume the following evolution:
	\begin{itemize}
		\item at time $n-2$, we have $X_{n-2} = 0$, $X^{(1)}_{n-2} = 1$
		\item at time $n-1$ only the source of interest transitions: $X_{n-1} = 1$, $X^{(1)}_{n-1} = 1$
		\item at time $n$ both sources transition: $X_{n} = 0$, $X^{(1)}_{n} = 0$
	\end{itemize} 
	Accordingly, slot $n-1$ sees the sole transmission of the reference source, so that $Y_{n-1}=1$, whereas a collision is experienced over slot $n$, i.e. $Y_n = \collision$. In this situation, the D\&H estimator outputs the sequence $\est_{n-1} = 1$, $\est_{n}=1$, providing an erroneous estimate in slot $n$ (i.e., $\est_n \neq X_n$) Conversely, the output of the threshold test on the APP logarithmic ratio in \eqref{eq:lambdan_def} performed by the MAP approach returns the correct estimates in both time instants. This can readily be verified by observing that, for the case under study, \mbox{$\mathsf P[X_{n}=0 \,|\, Y_n=\collision,Y_{n-1}=1,Y^{n-2}=y^{n-2}\,] = 1$}. Indeed, the observation of a collision implies that both nodes transmitted, and hence changed their state, providing certain knowledge of the state of the reference source at time $n$ as well. The suboptimality of the D\&H estimator stems by disregarding this type of information. 
\end{example}

To characterize the performance of this low-complexity solution, we focus on the average error probability $P_e$, which can be effectively computed by jointly tracking the source state and estimate processes via the Markov chain $(X_n,\est_n)$. The analysis we present is exact under random transmissions, whereas it resorts to the myopic surrogate model when the reactive strategy is implemented.

\begin{figure*}
	\centering
	\subfloat[random transmission strategy]{
	\includegraphics[width=.44\textwidth]{./figures/markov_DH_random.pdf}
	\label{fig:mc_est_random}
	}
	\hspace{-1.5em}
	\subfloat[reactive transmission strategy]{
		\includegraphics[height=.32\textwidth]{./figures/markov_DH_reactive.pdf}
		\label{fig:mc_est_reactive}
	}
	\caption{Markov chains $(X_n,\est_n)$ tracking the evolution of reference source state and D\&H estimate, in the case of a random (a) and reactive (b) transmission policy.}
\end{figure*}

Let us first focus on the random approach. In this case, the transition probabilities of the chain are summarized in Fig.~\ref{fig:mc_est_random}, where we recall that $\pup = \alpha (1-\alpha)^{M-1}$ is the probability that a node  successfully delivers an update over a slot. As an example, consider state $(X_n,\est_n)=(0,0)$. The process remains in the same state over the next slot if no change of state occurs, i.e. with probability $\qzz$. Note indeed that $\est_{n+1}$ will remain $0$ both in case of transmission and successful delivery of an update (i.e. $Y_{n+1}=0$), and in the absence of a received packet from the reference source (i.e. $Y_{n+1}\in\{\idle,\collision,\izero,\ione\}$). Instead, no transition to state $(0,1)$ can take place, since the D\&H estimator would only reset $\est_{n+1}$ to $1$ upon receiving an update from the source containing that value, which is not possible when $X_{n+1}=0$. In turn, the system moves to $(1,0)$ \--- providing an erroneous estimate of the source state \--- whenever the node of interest changes state (probability $\qzo$) but does not deliver an update, either due to a collision or for lack of transmission (overall probability $1-\pup$). Conversely, a transition to $(1,1)$ occurs when the source moves to state $1$ and successfully sends a packet in slot $n+1$ (probability $\qzo \pup$). All other probabilities in the chain can be derived following a similar reasoning.

The finite state Markov process is readily shown to be aperiodic and irreducible, and thus ergodic. Accordingly, the error probability $P_e$ introduced in \eqref{eq:Pe_def}, expressing the average time spent by the chain in $(0,1)$ and $(1,0)$, can be computed as the sum of the stationary probabilities of such states, denoted by $\pi_{(0,1)}$ and $\pi_{(1,0)}$. Solving the balance equation, we get 
\vspace{.3em}
\begin{align}
	P_e = \pi_{(0,1)} + \pi_{(1,0)} = \frac{2 \qzo \qoz \left(1-\pup \right) }{(\qzo + \qoz)\left[\,\pup + (1-\pup)(\qzo + \qoz)\right]}\,.
	\label{eq:Pe_DH_random}
\end{align}

\vspace{.3em}
The same approach can be leveraged to derive the performance of the D\&H estimator when the nodes operate following a reactive transmission policy, leaning on the surrogate myopic model introduced in Sec.~\ref{sec:myopicest}.  The corresponding transition probabilities for the Markov chain $(X_n, \est_n)$ take the form reported in Fig.~\ref{fig:mc_est_reactive}. In this case, the term $(1-\tilde\alpha)^{M-1}$ captures the probability for a source to deliver an update over a slot once a state change has taken place, with the activation probability $\tilde\alpha$ defined in \eqref{eq:myopic_def}. The stationary distribution of the chain gives in this case
\begin{align}
	\pi_{(0,1)} \approx \frac{\qoz (1-(1-\tilde\alpha)^{M-1})}{(\qzo+\qoz)(2-(1-\tilde\alpha)^{M-1})}, \quad 
	\pi_{(1,0)} \approx \frac{\qzo (1-(1-\tilde\alpha)^{M-1})}{(\qzo+\qoz)(2-(1-\tilde\alpha)^{M-1})}
\end{align}
leading to an average error probability
\begin{align}
	P_e \approx \dfrac{1-(1-\tilde\alpha)^{M-1}}{2-(1-\tilde\alpha)^{M-1}} \,.
	\label{eq:Pe_DH_reactive}
\end{align}
As discussed, this is exact for symmetric sources (i.e. $\qzo=\qoz$), whereas it is only an approximation in the asymmetric case. 

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{./figures/Pe_DH_symmetric.pdf}
	\caption{Average state estimate error probability, $P_e$, against the number of devices in the network, symmetric source case ($\qoz=\qzo=0.01$). Solid lines denote analytical results for the D\&H estimator, whereas circle markers the outcome of Monte Carlo simulations. Dashed lines report  results for a MAP estimator using \eqref{eq:PEMAPRAND} and \eqref{eq:PEMAPREACT}. Different colors indicate the performance attained under the random (blue) or reactive (red) transmission policy.} 
	\label{fig:Pe_symmetric}
\end{figure}

First insights on the behavior of the D\&H estimator are offered by Fig.~\ref{fig:Pe_symmetric}, which reports $P_e$ against the number of nodes in the network in the case of symmetric sources ($\qzo=\qoz=0.01$). Blue lines refer to performance attained under the random transmission policy, whereas red ones are representative of the reactive approach. In the former case, the activation probability has been set as the reciprocal of the number of nodes, i.e., $\alpha=1/M$, in order to maximize the throughput and thus the average number of delivered updates. In the plot, solid lines report the analytical results for the D\&H estimator obtained via \eqref{eq:Pe_DH_random} and \eqref{eq:Pe_DH_reactive}, whereas circle markers denote the results of Monte Carlo simulations. Finally, dashed lines  show the performance of a MAP estimator, which can be derived from the \ac{DE} analysis. In particular, for the random transmission strategy case the error probability is
\begin{equation}
 P_e = \lim_{n \to \infty} \sum_{\lambda_n \leq 0} P(\lambda_n,0) + \lim_{n \to \infty} \sum_{\lambda_n > 0} P(\lambda_n,1)   \label{eq:PEMAPRAND}
\end{equation}
where $P(\lambda_n,x_n)$  is computed with the recursion \eqref{eq:DErand}. Note that to practically estimate the limit in \eqref{eq:PEMAPRAND} it suffices to let $n$ grow large enough (e.g., $n\approx 10^5$) to observe converging probability estimates. Similarly, the error probability for the \ac{MAP} estimator for the reactive transmission strategy case can be obtained, in the myopic approximation setting, as
\begin{equation}
 P_e \approx \lim_{n \to \infty} \sum_{\tilde\lambda_n \leq 0} P(\tilde\lambda_n,0) + \lim_{n \to \infty} \sum_{\tilde\lambda_n > 0} P(\tilde\lambda_n,1)   \label{eq:PEMAPREACT}
\end{equation}
where $P(\tilde\lambda_n,x_n)$ follows from the \ac{DE} recursion \eqref{eq:DEreact}. 

The reported trends pinpoint a visible gap between the two estimators when few nodes populate the network. The rationale behind this goes along the lines of the discussion presented in Example 2. Indeed, while both MAP and D\&H attain an exact knowledge whenever a packet from the tracked source is received, the former refines its estimate also in the presence of an idle slot, a collision, or upon receiving a packet from another node ($Y_n\in\{\idle,\collision,\izero,\ione\}$). Such side information is especially beneficial for low values of $M$, as it allows to infer with a good level of confidence the state of the reference process. A simple quantitative intuition on this can be grasped by focusing on the reactive strategy and by considering the likelihood ratio 
\begin{align}
	\dfrac{\mathsf P[ X_{n} = X_{n-1}, Y_n = \collision \,]}{\mathsf P[ X_{n} \neq X_{n-1}, Y_n = \collision \,]} = \frac{(1-\alpha) \left[1-(1-\alpha)^{M-1} - (M-1)(1-\alpha)^{M-2}\right]}{\alpha\left[1-(1-\alpha)^{M-1}\right]}\,
	\label{eq:pColl_reactive}
\end{align}
obtained in the event of a collision and only looking at the outcome of the last slot. The quantity evaluates to $0$ for $M=2$, allowing the MAP estimator to extract exact knowledge on the change of state, as discussed in the previously presented example. 
Interestingly, the performance gap between the two approaches vanishes as the number of sources increases. For larger $M$, indeed, idle slots occur more seldom, and the impact of observing a collision on the MAP estimate of the reference source becomes weaker. A hint on this is again offered for the reactive case by \eqref{eq:pColl_reactive}, as the likelihood ratio converges to $(1-\alpha)/\alpha$ for $M\rightarrow\infty$. This observation is of practical relevance, suggesting that the simple D\&H solution offers good performance in sufficiently large networks when symmetric sources are to be tracked. 

Fig.~\ref{fig:Pe_symmetric} also reveals that a lower error probability is attained for the configuration under study when nodes implement a reactive transmission approach, especially for low to intermediate values of $M$. The choice of accessing the channel only to signal a change of state is in this case particularly beneficial, increasing the probability of successfully notifying an update. Conversely, when sources are sampled at random times, nodes may attempt to report information which is already available at the receiver, congesting the medium unnecessarily and generating additional collisions that reduce the estimator accuracy.

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{./figures/Pe_DH_asymmetric.pdf}
	\caption{Average state estimate error probability, $P_e$, against the number of devices in the network, asymmetric source case ($\qoz=0.01, \qzo=0.1$). Solid lines denote analytical results for the D\&H estimator, whereas circle markers the outcome of Monte Carlo simulations. Dashed lines report results for a MAP estimator obtained via \eqref{eq:PEMAPRAND} and \eqref{eq:PEMAPREACT} (myopic surrogate). Different colors indicate the performance attained under the random (blue) or reactive (red) transmission policy.}
	\label{fig:Pe_asymmetric}
\end{figure}


These remarks are complemented by Fig.~\ref{fig:Pe_asymmetric}, which shows the same set of performance trends in the case of asymmetric sources, assuming $\qzo = 0.01, \qoz = 0.1$. Within the plot, let us first consider the behavior observed when the reactive policy is implemented (red lines). In this case, simulation results show a very tight match with the analytical formulation of $P_e$ for the D\&H estimator \eqref{eq:Pe_DH_reactive}, obtained relying on the myopic surrogate approximation. On the other hand, a significant gap is present with respect to the behavior of a MAP approach, for all values of $M$.
This stems from the long time that may be required for an erroneous D\&H estimate to be corrected. For the configuration under study, for instance, a change of the Markov chain $(X_n,\est_n)$ in  Fig.~\ref{fig:mc_est_reactive} from state $(0,1)$ to an exact knowledge can occur at the earliest when the source takes the less likely transition to state $1$ and the transmitted update is correctly received (i.e., $(X_n,\est_n)$ transitions to $(1,1)$, taking on average $1/[\qzo(1-\tilde\alpha)^{M-1}]$ slots). Conversely, the MAP approach can better refine its estimate at each slot, possibly correcting the erroneous knowledge without the need for the source to perform any further transmission. 

In addition, and in contrast to what observed in the symmetric case, the D\&H estimator performs worse when nodes implement a reactive rather than a random transmission policy, already for relatively low values of $M$. The trend can again be explained observing that in the former case the estimator can remain in error for a long time due to lack of transitions (and thus update transmissions) of the reference source. When delivery attempts are performed at random times, instead, such periods of drought can be shortened, with beneficial effects on the average error probability. 


